Diffusing Your Mobile Apps: Extending In-Network Function Virtualization to Mobile Function Offloading

Motivated by the huge disparity between the limited battery capacity of user devices and the ever-growing energy demands of modern mobile apps, we propose INFv. It is the first offloading system able to cache, migrate and dynamically execute on demand functionality from mobile devices in ISP networks. It aims to bridge this gap by extending the promising NFV paradigm to mobile applications in order to exploit in-network resources. In this paper, we present the overall design, state-of-the-art technologies adopted, and various engineering details in the INFv system. We also carefully study the deployment configurations by investigating over 20K Google Play apps, as well as thorough evaluations with realistic settings. In addition to a significant improvement in battery life (up to 6.9x energy reduction) and execution time (up to 4x faster), INFv has two distinct advantages over previous systems: 1) a non-intrusive offloading mechanism transparent to existing apps; 2) an inherent framework support to effectively balance computation load and exploit the proximity of in-network resources. Both advantages together enable a scalable and incremental deployment of computation offloading framework in practical ISPs' networks.

==> revision.tex <==
\newcommand{\Revision}{474f74f}


==> sections/deprecated/cache.tex <==

%\subsection{Investigate Realistic App Market}
\section{In-Network Function Caching}
\label{sec:cache}

\rone{Although, the technique in identifying functionality overlap is rough and not very exact, it provides a ball park number. However, I had hard time linking the result/motivation to the rest of the paper. The evaluation does not show that popular classes can be offloaded. Instead, it uses two non-representative workloads. I wasn't sure how the benefit extends to many apps, as implied by the motivation in Section 3.}

\manote{We discussed doing a new plot with X-Axis number of popular apps and Y-axis cache size.}

\manote{Well there should be apps using the face detect apis, so it kind of does offload a common functionality. Perhaps we dont explicitly say its the Android official Face Detect API.}

\manote{Additionally we can try to add a new opensource app.}

\begin{figure*}[!htb] % not h only
\centering
\subfloat[Installation size of apps as a function of app popularity.]{%
\includegraphics[width=0.3\textwidth]{figures/caching/sizePerPopularity}%
\label{fig:install}%
}\hfil
\subfloat[Percentage of unique classes per app as a function of name depth used for comparison.]{%
\includegraphics[width=0.3\textwidth]{figures/caching/ClassespbpackageSimilarity}
\label{fig:uniqueclasses}%
}\hfil
\subfloat[Number of classes per app as a function of app popularity.]{%
\includegraphics[width=0.3\textwidth]{figures/caching/classesPerPopularity}%
\label{fig:popularity}%
}\hfil
%\subfloat[Obfuscated class name distribution.]{%
%\includegraphics[width=0.2\textwidth]{figures/caching/packageObfuscation.pdf}%
%\label{fig:packageobfuscation}%
%}\hfil
\caption{Study of over 20K Google Play apps regarding their size, structure and uniqueness.}
\label{fig:structure}
\end{figure*}

%%% Many questions arise from such requirement, e.g., \emph{what are the storage requirements for hosting an application? can we provide the majority of the most popular apps? Is it possible to reduce the needed cache size?} 
A key insight that informs the design of INFv is the potential of network functionality caching.
In this section we give some intuition behind the idea and empirically show its feasibility via a study of over 20K of the most popular apps on the Google Play Store in February 2016.
%Caching offloaded functions in a network leads to a natural question -- what would be the storage requirement for INFv? To answer this question, 
% performed a study over 20K most popular apps on the Google Play Store in February 2016. %(i.e., parsing \texttt{smali}\footnote{Androids' disassembled bytecode syntax as outputted by apktool} files).
%%% Note that the top 1\% of most downloaded apps account for over 81\% of the total downloads~\cite{Viennot:2014} (November 2013). Since our dataset covers over 1.3\% of the market\footnote{Google Play had 1.5 Million apps in the first quarter of 2015\cite{appbrain}}, we consider it as a representative sample. 
In summary, our investigation reveals two important facts: 1) a very small amount of apps account for most of the downloads; 2) there is a significant code overlap due to commonly used libraries. Two facts together indicate a medium storage requirement on INFv as the detailed analysis shows in the following.

Fig.~\ref{fig:install} shows that the distribution of the installation size of mobile apps has a $\mu \approx 23.9MB$ (mean), $\tilde{x} \approx 10.2MB$ (median) and $\sigma \approx 66.9MB$ (standard deviation). 
By comparing to the numbers reported in \cite{Viennot:2014}, we also confirm that $\approx 15,000$ apps are responsible for 81\% of all Google Play downloads and in total they require an aggregated storage of 409~GB. %%%, considering an installation size of 27MB (3rd quartile). 
%\manote{its the total aggregate space. Up to is due to poing 1 below.}
This is apparently a manageable size even without excluding a few outliers which are up to 2.1~GB. %Moreover, it also justifies the sample we used is a representative one.\jbnote{this comes out of no where, use a forward ref or something?}
%%% are responsible for big chunks of storage, but could this be reduced if apps share functionality?
%The following two facts can reduce the storage requirement even more: 1)~most mobile offloading architectures offload only partitions of the app (often removing heavy app assets/resources), 2)~we have also found that apps tend to share a significant amount of functionality. 

%To answer this question we need to understand apps structures.
%%% In Android, app functionality (e.g., classes and methods) is organized in packages, an abstraction similar to directories/folders in common file systems. Packages can contain functionality and/or other packages.
%%% Android apps organize functions into packages which are further identified with a hierarchical naming scheme similar to domain names.
%%% Any given package name includes all the parent package names separated by dots
%%% The hierarchy is measured with depth as Java naming convention~\cite{packagenames} (e.g., ``\texttt{com.facebook.katana}'' has a package depth of 3).
%%% These tend to follow the Java naming convention: a top level domain (``\texttt{com}''), company name (``\texttt{facebook}''), application name (``\texttt{katana}'') and optionally a region.
%%% Packages provide valuable help in grouping functionality %(which include the containing package name)  and are core to the routing mechanisms of offloading systems to locate the remote functionality to execute.
% and for profiling apps.
%%% Detecting shared functionality across apps should be as easy as detecting functionality with the same name.
 %A package with 4 names (i.e., package name depth of 4) is likely to be sufficient for distinguishing different functionality across applications even within the same company.
%They can also be used to detect functionality overlaps in apps which reuse common libraries.
INFv exploits the large overlap in app functionality to intelligently cache functionality in the network \manote{we do not mention how}.
To understand why and how this is possible, a brief overview of Android app organization and packaging is necessary.
Android apps organize functions into packages which are further identified with a hierarchical naming scheme similar to domain names.
Intuitively, the hierarchical naming could facilitate us in identifying shared functionality across apps.
Unfortunately, naming in Android can be affected by obfuscation, a security mechanism that remaps functionality and package names.
It makes it hard, if not impossible, to detect similarities based on simple name comparisons.
E.g., a package ``\texttt{com.apple}'' from app A and a package ``\texttt{com.google}'' from app B can both be renamed to ``\texttt{a.a}''.
%\subsection{App dataset}
%\subsubsection{Dataset}
%\label{sec:dataset}
%Obfuscated package names are typically small (e.g., \texttt{a.b.c}) and their per-package-depth names are often represented by a single character (e.g., attributed in an alphabetical order from a-z).
But, since in Android obfuscation (i.e., Proguard) names are attributed alphabetically, we found that it is possible to detect if a package name is obfuscated or not based simply on name length.
We found that 37.5\% of apps have potentially obfuscated packages with name ``a'' (at any given depth), while 82\% of the apps have at least one class named ``a''.
%Many package names are often not obfuscated, such as names referenced from the application manifest and many third-party library packages.
%As shown in Figure~\ref{fig:packageobfuscation}, f
By studying the name distribution with a single character at any given depth, we have found that the majority of obfuscated package names tend to have names between ``\texttt{a}'' and ``\texttt{p}''.
This means that, for the apps in our dataset, \emph{a simple filter to find packages names which have, at any given depth, a name with just one character is enough to ignore the majority of obfuscated packages (8\% of all packages).}%\jbnote{I really don't know what this means, especilly considering the next two lines...} 
%Note that, while depth 9 and 10 seem to have a relatively high number of obfuscated packages (close to 10\% for the latter), this is exacerbated by the low number of packages with such depths.
%Unfortunately functionality (class) names do not follow such a distribution and often have names with two or more characters.
%Therefore using a filter based solely on their names could produce many false positives and discard valid names.

%With the naming limitations in mind, 
We have used the package names to estimate functionality similarity. 
If the same package name exists in two different apps we consider the functionality within this packages to be similar.
Obviously, if we look at low depth names ($N < 3$), such as the first depth packages (e.g., ``\texttt{a}'' in ``\texttt{a.b.c}'') which contain all other packages and functionality, many apps are likely to share the same name and therefore, most of the functionality will be considered similar (false positives).
If we look deeper into the package hierarchy, however,  we can greatly reduce the rate of false positives.
% as these package names tend to include the app and owner names (e.g., ``\texttt{com.facebook.katana}''). \jbnote{I don't know what the rest of this sentence means}
%Understanding how functionality overlaps across different apps can help us refine the storage requirement.
%%% liang: I am thinking to move it somewhere else .... maybe into other sections. 
%%% Since we are interested in functionality reuse (not cloning), e.g., use of third-party libraries, and due to obfuscation limitations, we estimated class uniqueness based on the package they occur. To overcome obfuscation we performed a market study and created a simple filter to ignore potentially obfuscated packages, our technique contributes to analogous research (Section \ref{sec:related}) and is described in Section \ref{sec:obfuscation}.
Fig.~\ref{fig:uniqueclasses} shows the percentage of unique classes per app based on a comparison on their first N package names. %as a function of package name depth. %(e.g., ``\texttt{a.b.c}'' has a package depth of 3).
%\jbnote{Need some explanation of what package names are and why they can be useful in this analysis}
%We compared package names based on their 1-N depth package names.
The number of unique classes are calculated as the \emph{total number of classes} in the app minus the number of classes belonging to \emph{non-obfuscated} package names that also exist in at least one other app.
%We note that 
% whose first-N package names are found in more than one app.
% I.e., the number of classes in the app minus the number of classes who also appear in at least one other app. 
%Package comparison is based on the name depth considered in the x-axis.
%A N-depth package includes the classes of a child $(N+1)$-depth package.
%Comparisons on a low depth (e.g., $N < 3$) mean that most of the packages will be considered similar (e.g., ``\texttt{a.b}'' is considered the same as ``\texttt{a.d}''), 
Considering that the package name distribution has $\mu \approx 4.7$, $\tilde{x} \approx 5.0$ and $\sigma \approx 1.6$, and that most package names have a depth between 4 (Q1) and 6 (Q3), even if we do a conservative comparison of packages based on their first 5 name depths (50th percentile), we can see that \emph{only 47\% (mean) of apps' classes are unique}.
Note that while higher values ($N \geq 8$) reduce false positives, they also increase the number of false negatives as classes within packages with smaller depths are considered as unique. %as packages with such depth fall outside of the standard deviation of the package name distribution\jbnote{huh?}.
If we consider a depth of 4, which is likely to include the name of the app and respective developer (e.g., ``\texttt{com.facebook.katana.app}''), we see that 75\% (median) of apps' functionality is common with at least one other app.
The analysis thus indicates that it is safe to conclude that there is a substantial overlap between app functionality in the Android ecosystem.
% According to the naming conventions a package depth of 4 should already suffice to differentiate functionality, this value can potentially be as high as 75\%.
%we can see that for these depths \emph{only up to 26-75\% (mean values) of apps' classes are actually unique to the app itself}.
%In practice, as Android apps' package names should follow the Java naming conventions~\cite{packagenames}, a package depth of 4 is likely to be sufficient for performing comparisons as it should already provide information regarding the package developer and the app name (i.e., a top level domain, e.g., ``\texttt{com}'', company name, e.g., ``\texttt{facebook}'', application name, e.g., ``\texttt{katana}'' and optionally a region).
%Fortunately, in most cases a package depth of 4 should suffice to distinguish functionality and even if we choose the more conservative comparison using the 50th percentile, i.e., package depth of 5, we can see that \emph{only up to 47\% (mean) of apps' classes are unique}.

This significant overlap in functionality provides a unique opportunity for deployment in a modern ISP network.
By co-locating common functionality, we can reduce the storage requirements while at the same time allowing us to exploit the network topology to ensure that functionality is available as close to users as possible.
The design and architecture of INFv is informed in large part by this insight.

% We leverage this fact 
% Since there is a significant overlap and since we expect the caching cost to be mostly due to functionality (i.e., no app assets such as images), we believe that if these apps are co-located their storage space can be greatly reduced.
%As mobile code offloading architectures already tend to partition apps, our investigation in the realistic App market provides strong supportive arguments for function offloading. Since apps share a large amount of functionality, the costs of caching and hosting functionality partitions can be greatly reduced.


==> sections/deprecated/motivation.tex <==
\section{Motivation}
\label{sec:motivation}

\liang{section need to rewrite}
INFV is motivated by two aforementioned observations. The first one (on abundant in-network resources) can be easily validated by noticing the strategic moves of big telecommunication companies. Namely, the current ISP infrastructure is transforming into NFV-enable network step by step quickly to improve utilisation rate\cite{telefonica:nfv,telefonica:cartablanco,telefonica:unica}. In this section, we validate the second observation by performing a deep investigation in current mobile application market. We focus on Android platform in this paper, how to generalise to other platforms like Apple's iOS will be discussed in Section \ref{sec:discussion}.

\begin{figure*}[htp] % not h only
\centering
\subfloat[Packages per app]{%
\includegraphics[width=0.3\textwidth]{figures/caching/PackageLevelDistribution.pdf}%
\label{fig:packagesperapp}%
}\hfil
\subfloat[Unique classes (\%) per app]{%
\includegraphics[width=0.3\textwidth]{figures/caching/PercentageOfNonUniqueClasses.pdf}%
\label{fig:uniqueclasses}%
}\hfil
\subfloat[CDF of the jaccard indexes for pairs of apps based on their packages. Each line represents a different package depth.]{%
\includegraphics[width=0.3\textwidth]{figures/caching/JaccardCDF.pdf}%
\label{fig:classespopularity}%
}
\caption{Study of the number packages and number/uniqueness of classes per application.}
\end{figure*}

3) Diffusing and hosting functionality on the network raises multiple challenges and these are exacerbated if we consider that this functionality is transparently transfered to the network.
One of these challenges relies on the multitude of different applications present in mobile app markets (e.g., 1.5M apps in the Google Play store\footnote{1st quarter of 2015 - http://www.appbrain.com/stats/number-of-android-apps}), each possibly composed by thousands of classes with variable number of methods\footnote{As both iOS and Android are object-oriented, we consider methods to be the closest match to the NFV function abstraction.}. 
Concerns are therefore raised regarding the caching capabilities of such system:
\begin{itemize}
\item How big are applications? \manote{no numbers on this yet, but should be extremely fast!}
\item What to partition app functionality? How to to version and update this functionality?
\item Can caching cost be reduced? Is there an overlap of functionality across apps?
\end{itemize}  

To answer these questions we have crawled the Google Play Market to download over 18K of the most popular free apps and decompiled them in order to perform static analysis.
We found (Figure~\ref{fig:classespopularity}) that, although applications can have considerable high number of classes (up to 25K), the 25th-75th percentile of apps have less than 10K classes.
This holds true independently of the number of downloads of the app, as we have also observed that apps with more downloads tend to have more classes.

In order to diffuse methods in the network and maintain some mechanism for updating these methods we require some sort of versioning.
When a client wants to execute a function in the network, he would provide the name schema for the function (e.g., function name) and a version identifier.
Tracking identifiers on a per method basis could be costly due to the high number of methods per application.
A reasonable solution consists on devising a grouping schema to functions.
Keeping the OO abstraction this grouping could potentially be done on a per class, package or application basis.
We argue that a per package basis can already be too coarse granularity as the number of classes can be orders of magnitude bigger than the number of packages, meaning that a single class update would require a whole package update.

In OO languages methods typically operate over some state, not only input variables and static state, but also their respective class state.
Class methods are also likely to share the same state and make intra-class method invocations.
Therefore, while different granularities might also have some advantages, we will consider class granularity as it can have a positive impact on state shattering, cost of communication between methods and a smaller impact on the cost of version tracking and respective delta updates.

Hosting an arbitrary number of app functions in the network can be costly, therefore it would be interesting to detect if there is an overlap of app functionality that could amortize this cost.
To do so, we collected all app's packages and respective class count.
Packages were grouped based on their depth, for example \texttt{a.b.c} has a depth of 3, while \texttt{a.b} has a depth of 2.
We note that the number of classes of the second includes the classes of the first.

\begin{figure*}[htp] % not h only
\centering
\subfloat[Popularity distribution of common packages (e.g., ads, rendering, networking)]{%
\includegraphics[width=0.3\textwidth]{figures/caching/packagesPerApp.pdf}%
\label{fig:packagesperapp}%
}\hfil
\subfloat[Another figure for "Similarity vs. popularity"?]{%
\includegraphics[width=0.3\textwidth]{figures/Placeholder.png}%
\label{fig:uniqueclasses}%
}\hfil
\subfloat[\# of classes vs. popularity]{%
\includegraphics[width=0.3\textwidth]{figures/caching/classesPerPopularity.pdf}%
\label{fig:2}%
}
\caption{Study of the number packages and number/uniqueness of classes per application.}
\end{figure*}

The plots in Figures~\ref{fig:packagesperapp} and \ref{fig:uniqueclasses} depict, respectively, the distribution of packages and the percentage of unique classes per application, depending on the considered package depth.
Considering a depth of 1 means that packages such as \texttt{a.b} and \text{a.c} will be ignored and only their aggregated class count is considered (i.e., package \texttt{a}).
For the sake of simplicity, we assume that classes within a similarly named package across two applications are similar.
We consider this to be a reasonable assumption since most libraries/apps tend to have custom package naming related to their app, developer and company names.
Since for lower package depth these names will have more collisions, the higher the package depth considered, the most likely the class similarity assumption is to be held true.
To make our assumption more conservative, the total number of unique classes is calculated as the total number of classes in the app (independently of package depths) minus the number of classes belonging to packages which the N-depth package name is shared by at least one more app.   

As shown in Figure~\ref{fig:uniqueclasses}, as expected, for a depth of 1, apps are likely to have no unique classes as most tend to share the 1-depth package name (e.g., \texttt{com}).
If we look at rather deep package name depth of 5, which will be less likely to collide (e.g., \texttt{a.b.c.d.e} and \texttt{a.b.c.d.f} would be considered different packages), it not only possesses an higher median and average number of package counts (Figure \ref{fig:packagesperapp}), but we have also found that the median and average count of unique classes are around 40\% (Figure \ref{fig:uniqueclasses})\manote{check the exact number}.
This is a very clear indicator that \emph{apps tend to have an high number of shared classes which are not app specific}.
In figure \ref{fig:packages} we show an example of the packages (we ignored compatibility/OS packages such as android support) present in the most number of apps. 
We can see that there are 3rd-party library packages that are present across high percentage of apps.
While the two first are Google technologies, such as google play services and ads, we see that Facebook libraries are present in more than 30\% of the apps.
These libraries also include rendering and animation packages (e.g., unity3d and nineoldandroids).

\manote{Note to self: check obfuscation and package depth for upcoming plot}

5) Server-assisted mobile application execution can provide support for computation intensive applications/services (e.g., aggregation of sensor data flows, voice processing, 3D rendering, etc), for which, executing the computation remotely can greatly reduce its energy costs even in the presence of extra communication.
Mobile remote execution has been the topic of multiple research works~\cite{chun_clonecloud:_2011,chen_coca:_2012,gordon_comet:_2012,kemp_cuckoo:_2010,cuervo_maui:_2010,zhang_refactoring_2012,kosta_thinkair:_2012}. 
For example, CloneCloud~\cite{chun_clonecloud:_2011} performed experiments with a virus scanner, face detection and web page categorization, achieving up to 20x execution speed-up and a 20-fold decrease of energy spent.
Aggregation of data and remote storage are also possible use cases as these devices often have limited storage capacity.
When providing remote resources, there needs to be a balance between the energy cost of the extra communication induced by the remote execution and the benefits of providing these remote resources. 
Therefore, proximity and latency have a relevant impact on such architectures and can reduce the scope of applications/services
they can provide, for example, delay-sensitive and interactive applications. 
Latency also increases the energy consumption in mobile devices as having a longer established communication channel in mobile networks is expensive \manote{trinity refs here}. 
Having higher communication energy costs can often become a no-go even for non-interactive or delay-sensitive computation intensive applications.
Therefore, by adopting the NFV paradigm, not only these architectures could be applied to more apps but also perform better.

\manote{would it be possible to show: other architectures if the user moves to somewhere with higher latency the code is no longer offloaded, while our functionality moves closer to the user, eventually offloading methods again?}


%\manote{Another strong case for offloading technologies is to reduce the costs of online presence. \cite{Aucinas} shows how popular\'s app background activities such as maintaining online presence can have severe impact on the device energy consumption (up to nine times faster battery drain). 
%Although Android provides the Google Cloud Messaging (GCM) to provide push notifications and reduce background network usage, apps often use their own communication channels. For example, Facebook makes use of a pub/sub MQTT protocol which is not shared across its multiple apps (e.g., main app and messenger), doubling the cost of maintaining connectivity. 
%If online presence functions are offloaded, their connectivity cost can be reduced by multiplexing traffic through a single channel. 
%Another aspect of background activity is that it often has no impact on user experience.
%For example, applications often use ad libraries that wake up the device often (cite alarms paper), running such functions on the cloud could avoid waking the device while still maintaining their functionality once the mobile resumes.}


==> sections/deprecated/newmotivation.tex <==
\section{Motivation}
\label{sec:motivation}

% \begin{table*}[htp]
% \centering
% \begin{tabular}{|l|l|l|l|}
% \hline
% Name       & Granularity                                                    & Profiling                                                                          & Partitioning        \\ \hline

% MAUI~\cite{cuervo_maui:_2010}      & Method                                                         & \begin{tabular}[c]{@{}l@{}}Exec. time, State, Energy \& Network\end{tabular} & Manual (Annotations)                    \\ \hline

% CloneCloud~\cite{chun_clonecloud:_2011} & \begin{tabular}[c]{@{}l@{}}Thread (method)\end{tabular}      & \begin{tabular}[c]{@{}l@{}}Exec. time, Network \& Energy\end{tabular}          & Automated (Offline)                                                          \\ \hline

% ThinkAir~\cite{kosta_thinkair:_2012}   & Method                                                         & \begin{tabular}[c]{@{}l@{}}Exec. time, Network \& Hosting cost\end{tabular}    & \begin{tabular}[c]{@{}l@{}}Manual (Annotations)\end{tabular} \\ \hline

% Zhang et al.~\cite{zhang_refactoring_2012}        & Class (method)                                                 & \begin{tabular}[c]{@{}l@{}}State, CPU, Network \& Energy\end{tabular}                     & Automated (Offline)                                  \\ \hline

% Comet~\cite{gordon_comet:_2012}     & \begin{tabular}[c]{@{}l@{}}Thread (instruction)\end{tabular} & Execution time \textgreater 2RTT                                                   & Automated                                               \\ \hline

% \end{tabular}
% \caption{Mobile Code Offloading architectures based on their granularity, profiling metrics and partitioning strategy.}
% \label{tab:offload}
% \end{table*}


INFV is motivated by two aforementioned observations: there is a clear gap between battery capacity and the growing energy consumption of modern mobile applications~\cite{oliner_carat:_2013, Aucinas:2013:SOW:2535372.2535408}; and ISP networks are shifting towards the deployment of in-network multi-core general purpose machines following the NFV paradigm.

While Cloudlets~\cite{satyanarayanan_case_2009} discussed the impact of low latency in mobile code offloading and proposed the deployment of physically proximate decentralized clusters, similar to the abstraction of NFV, most of the more recent mobile code offloading architectures still rely on a mobile-to-cloud paradigm~\cite{cuervo_maui:_2010, kemp_cuckoo:_2010, kosta_thinkair:_2012,chen_coca:_2012, zhang_refactoring_2012, gordon_comet:_2012, chun_clonecloud:_2011}.
Furthermore, they cannot be directly applied in an ISP network since none has been designed to exploit network topologies let alone inherent load-balancing functionality.
Additionally, they tend to propose intrusive models that require either custom OS distributions~\cite{chun_clonecloud:_2011,gordon_comet:_2012}, app repackaging~\cite{zhang_refactoring_2012} and/or custom app distribution stores, greatly reducing their possible device adoption.
These observations naturally lead to an attempt on leveraging \emph{existing} in-network resources for dynamic offloading functionality from stock mobile devices to a network in order to improve both battery life and latency.
However, considering there is a huge amount of mobile apps on the market, an important question remains unanswered -- is it possible to accommodate all the offloaded functionality in an ISP network? 
Answering such questions requires investigation of real app markets and, while this has been mostly overlooked in previous research, we aim to shed light to these questions in this paper.

% \begin{itemize}

% \item App popularity is highly skewed, ...? is responsible for ...? downloads.

% \item There is a significant code sharing between different apps thanks to the commonly used library.

% \item The energy consumption of different apps is highly skewed. There is a small amount of apps responsible for most batter uses.

% \end{itemize}

% Consequently, a very conservative estimate based on our measurements indicates INFV needs ??? GB in-network storage to accommodate offloaded apps. In the following, we briefly present our measurement results.

%%% The first observation has been validated by a series of measurement work \cite{???} to show there are abundant in-network computation resources. Indeed, current ISP infrastructures are transforming into NFV-enabled networks to improve utilisation rate~\cite{telefonica:nfv,telefonica:cartablanco,telefonica:unica}\jbnote{I'm not sure I buy this by just saying that networks are starting to use NFV stuff... Where is the evidence that the boxes are being underutilized?!}.

%%% For the second observation, i.e., disproportionate app energy consumption, Oliner et al.~\cite{oliner_carat:_2013} show power hogging apps are responsible for 41\% degradation of battery life on average. Moreover, this percentage likely represents a \emph{lower} bound on the actual situation. Other studies~\cite{Aucinas:2013:SOW:2535372.2535408} have reported that a set of four popular apps can drain mobile device energy up to nine times faster. By offloading such power hogs, we can potentially reduce energy consumption by an order of magnitude~\cite{chun_clonecloud:_2011, cuervo_maui:_2010}. Furthermore, this does not only apply to the 10\% of apps that are computationally intensive apps~\cite{oliner_carat:_2013}; many normal apps (about 50\%~\cite{almeida_empirical_2016}) performing delay insensitive background tasks also consume a significant amount of energy due to CPU and data usage~\cite{Aucinas:2013:SOW:2535372.2535408} making them good candidates for offloading.

%% Automated mobile code offloading architectures typically partition apps based on energy consumption, used state, and execution time of each functionality.  The offloading decision is typically made during runtime and the network properties (i.e., latency/RTT times) are usually the determinant factors.
%%% Therefore the potential benefits of functionality offloading and their coverage are a factor of the systems latency. For example, Cloudlets~\cite{satyanarayanan_case_2009} proposed to exploit physically proximate decentralized and widely dispersed clusters of multi-core computers to achieve low latency. However, most mobile code offloading architectures still rely on a mobile-to-cloud paradigm~\cite{cuervo_maui:_2010, kemp_cuckoo:_2010, kosta_thinkair:_2012,chen_coca:_2012, zhang_refactoring_2012, gordon_comet:_2012, chun_clonecloud:_2011}.

%%% Even though we focus on Android platform in this paper, we will show how this framework can be equally applied to other platforms like Apple's iOS in Section \ref{sec:discussion}.


%%% In this section, we validate the second observation by performing a deep investigation of the mobile application market. We focus on Android in this paper, but generalizing to other platforms like Apple's iOS will be discussed in Section~\ref{sec:discussion}.





==> sections/deprecated/old_architecture.tex <==
\section{Partition and Profiling}
\label{sec:profiling}

\jbnote{There is so much crap in this and the previous section.. I'm not sure if it's really necessary. It gets cumbersome to read..}

% While we already addressed the design requirements and high-level architecture of INFv in the previous section, here we will discuss the implementation details and how we addressed some of its design challenges.

In this section, we discuss the implementation details of the architecture presented in Section~\ref{WHATEVER}, focusing specifically on how we addressed the outlined design challenges.

%Granularity: the question is function offloading will happen at what granularity? What is the trade-off between finer- and coarser granularity? We chose class-level granularity, how can we justify our design choice? E.g., each App on average has over 60,000 classes and each class has a set of well-fined applications which often depends on each other. Therefore, given a function might call other functions in the same class with high probability \liang{[probably show some stats based on statistic analysis]}, operations at class level can avoid unnecessary remote calls to further reduce communication overhead. Moreover, the class size is usually small so offload overhead is also small. 

In mobile code offloading, apps are typically partitioned into a set of functionality to execute locally and another to execute remotely.
Such system needs to detect good candidates to offload, e.g., based on energy consumption and execution time.
The selection is done via static and dynamic analysis on apps' behaviors (a.k.a., profiling apps).
%To assure that offloading an app does not consume more energy or takes longer than executing locally, apps need to be profiled.
Since profiling per se is energy consuming and can degrade devices' performance, we devise our first requirement:
\textbf{Req1)} \emph{App profiling should have minimal impact mobile device energy consumption and performance.}
In our design most of the profiled metrics and estimations are performed remotely (INFv servers) for a given mobile device.
%in INFvs' servers and the respective results are shipped to the devices in order to estimate the local parameters (i.e., execution time and energy consumption) required for offloading.

%Adittionally app analysis is also responsible for detecting functionality that should be executed locally and to approximate the existing estimations to the observed 

INFvs profiling subsystem consists of an app analysis cluster and repository containing these apps' partition functionality as well as their respective metadata.
This metadata includes the app representation (e.g., information regarding app structure and method invocations) and estimated resource usage (e.g., energy, execution time).
The app analysis cluster has a set of schedulers that launch VM instances to analyze apps then stores the respective results in the repository.
App analysis is done through static (i.e. parsing decompiled bytecode) and dynamic analysis of the apps.
% to retrieve functionality execution time, parameter state and energy consumption.
The first is used to retrieve the metadata app representation and do an initial prediction of possible partitions (e.g., pinning to execute locally functionality that uses devices hardware).
The second is used to benchmark app partitions and to retrieve functionality execution time, parameter state and energy consumption (i.e., partition's metadata), which is used for performing informed offloading decisions.


\subsection{App Partitions}
\label{sec:partitions}
%As we have discussed in Section \ref{sec:profiling}, 
App partitions describe sets of functionality to be executed locally or remotely.
In INFv we differentiate between partition functionality and metadata.
The latter including a representation of the app and the resource estimates for performing informed offloading decisions.
%In this section we will discuss our decisions regarding the offloading granularity (i.e., units of functionality to be offloaded) and the partitioning of apps based on the selected granularity.
%\subsubsection{Granularity}
%As seen in Table \ref{tab:offload}, o

Offloading can occur at multiple granularities (i.e., units of functionality to be offloaded).
%To this end there are multiple granularity levels at which offloading is possible.
The most common are method~\cite{cuervo_maui:_2010,kemp_cuckoo:_2010,kosta_thinkair:_2012,chen_coca:_2012} and thread~\cite{chun_clonecloud:_2011,gordon_comet:_2012} granularity.
The latter often incurs an extra cost of synchronization (e.g., thread state, virtual state, program counters, registers, stack, locks, etc), while still being restricted to method entry and exit points~\cite{chun_clonecloud:_2011}.
In order to better integrate with the NFV abstraction, our solution is based on method offloading.

Since most mobile architectures (e.g., iOS and Android) apps are developed in class-based object-oriented languages\jbnote{is this true for Objective-C?}, when possible we try to use a class offloading granularity.
Although each granularity has pros and cons, class granularity has some clear benefits regarding both number of invocations and state synchronization.
First, class methods are likely to invoke other methods of the same class, and secondly, these methods also likely to share common class state (e.g., class fields)\jbnote{Do we have any justification for statement?}. 
\manote{some stats here: number of classes per app, probability of a class method calling a method of the same class, probability of accessing class fields}
Typically, due to the object-oriented design, there are also better chances that class granularity will provide better semantic separation between application methods, and as we have seen in Figure~\ref{fig:uniqueclasses}, there is a large overlap of common classes and packages across apps, which minimizes the impact of storing app functionality in the network. 


\subsubsection{Opensource App representation \& analysis}

Our app representation (and its static analysis tool) is open-source\footnote{https://bitbucket.org/aknahs/droidbroker}.
It includes the information required to instrument the app, such as app starting points (as described in the manifest, e.g., activities, broadcast receivers, etc), the class methods and their inner invocations (represented through a graph). 
Similarly to DPartner~\cite{zhang_refactoring_2012}, it is also able to tag functionality based on the APIs they use.
This becomes particularly useful when we try to avoid offloading functionality that should execute on the device (e.g., sensors). 
It also contains structures for static and dynamic analysis information (e.g., occurrences and execution time), as well as graph visualization support (e.g., Gephi) to provide visual information regarding the clustering of functionality.
Using the representation of the app, INFv is able to check what are the entry and exit points of each of the classes/methods (e.g., graph edges for method invocations) of the partition in order to intercept their execution.
As Android applications have restrictive heap sizes (e.g., 48MB in Samsung Galaxy S2), our application representation has to be as small as possible.
%By analyzing the top 30 market apps (May'15) we determined that their average size is around 24MB.
%We measured the heap memory usage before and after loading our apk representations.
%In order to provide 
With the minimal information needed by the offloading mechanisms (e.g., how do classes interact), our uncompressed representation requires on average 3MB per app (based on the top 30 apps of our dataset).

\subsection{Partitioning}

In systems with class or method granularity, app partitions are typically done offline and require repackaging of the app.
% (except for Comet \cite{gordon_comet:_2012} and CloneCloud \cite{chun_clonecloud:_2011} which have custom Android distros).
In such cases, although some support multiple partitions for the same app, the partitioning cannot be done dynamically after app installation.
This means that if the app behavior (dependent on user interaction) differs from the behavior observed during the partitioning process and there is no partition that satisfies the new use case, the system cannot adapt properly.\liang{I guess you mean the consumption model within an app has changed ... so needs repartition?}\manote{Functions receive arguments that are sometimes defined by users. Imagine that the app is tested with an automated input generator. What if this input is not representative of the user. What if users have different patterns. We dont know if there will be significantly different energy patterns}
App-repackaging can also be a barrier to implementing automated profiling through UI instrumentation (such as the one used in~\cite{chun_clonecloud:_2011}).

\emph{In INFv apps are not repackaged and new partitions can be defined/loaded at any point in time} using a custom class loader, details of which appear in Section \ref{sec:instrumentation}.
Partitions in INFv are represented by the partition functionality, which is hosted at the network nodes, and partition metadata which is fetched by the mobile devices.
Partition metadata includes lists of classes and a set of parameters used for performing offloading decisions (e.g., estimated energy, execution time, state, etc).
The INFv monitor (Figure~\ref{fig:architecture}) will use the partition's metadata to decide which methods to intercept (exit and entry points of the partition) and potentially offload.
%While not the main focus of this research, we implemented an app analysis system (which we used in Section \ref{sec:motivation:preliminary}) that produces graph-based partition representation model for which it should be fairly simple to map existing class granularity partitioners, such as DPartner~\cite{zhang_refactoring_2012}. 
Previous research has focused on the challenges of performing app partitioning with class granularity and it should be fairly simple to map existing partitioners, such as DPartner~\cite{zhang_refactoring_2012}, to our system.
That said, some of the limitations of the existing partitioners and the security/overhead of the interception mechanisms are discussed in Section~\ref{sec:discussion}, while in Section~\ref{sec:evaluation:linpack} we will discuss the impact of different partitioning choices in the energy consumption and execution time of our offloading architecture.

\subsection{Profiling}

The energy and execution time of apps is dependent of many variables (e.g., connectivity type, screen state, idle) and offloading can often increase energy consumption and execution time depending on these variables.
To prevent such cases, mobile code offloading architectures need to be able to defer offloading functionality when it is estimated to perform worse than executing locally.
%Literature tends to profile multiple metrics (e.g., execution time, state, energy, network usage, cpu cycles) to aid this decision.
%In order to define each partition parameters, the values of their energy, execution time and transmission state need to estimated.
App profiling can aid in such decisions, but it also incurs a significant overhead in energy and execution time.
Mobile devices have limited heap sizes and tracing app functionality can often make apps unresponsive.
%This can be overcome by performing coarser profiling (e.g., process level) and/or choosing memory oriented heuristics to monitor smaller subsets of functionality.
While monitoring subsets of likely ``heavy'' functionality based on static analysis~\cite{zhang_refactoring_2012} (e.g., code loops, similarity clustering) could reduce this cost, these partitions still need to be profiled over time. Furthermore, many of the class/method relations used for selecting subsets (e.g., semantic similarity \cite{zhang_refactoring_2012}) are affected by the obfuscation patterns of apps (discussion in Section \ref{sec:obfuscation}).

Instead of profiling functionality on the mobile device, INFv provides an app analysis backend (depicted in Figure \ref{fig:architecture}), in which apps are instrumented using UI automation mechanisms (pseudo-random input events \cite{monkey}).
For each application an execution time and power model is derived depending on different metrics (e.g., network, cpu frequency).
The backend is heterogeneous and composed by x86 and physical mobile devices, which we use to derive energy models.
We rely on a similar model to the one proposed by PowerTutor \cite{zhang_accurate_2010} to predict energy consumption, which loops through different device power states separately to derive a power model through regression.
It can accurately (0.8\% on average) estimate energy consumption with a low error (at most 2.5\%).
While automated input generation might not cover all app code, there has been a significant amount of research towards providing better code coverage \cite{machiry_dynodroid:_2013,mahmood_evodroid:_2014}.

\section{Transparent Offloading}
\label{sec:offloading}
\subsection{Runtime instrumentation}
\label{sec:instrumentation}

Once INFv fetches the partition metadata, it requires mechanisms to extend applications' functionality in order to support the offloading of the partition classes.
In previous literature these mechanisms were based on specialized programming frameworks and annotations \cite{kemp_cuckoo:_2010,chen_coca:_2012,kosta_thinkair:_2012,cuervo_maui:_2010}, app repackaging or by extending OS capabilities.
In many OO languages, adding additional behavior without altering the original application code can be accomplished with Aspect Oriented Programming (AOP), which has been explored in recent work \cite{zhang_refactoring_2012}.
Unfortunately this solution requires a specialized compiler (e.g., AspectJ compiler) and application repackaging.
This raises a challenge of distributing these repackaged apps, potentially requiring custom app stores or repositories.
Another solution is to provide a custom firmware \cite{gordon_comet:_2012}, which we want to avoid in order to support more devices.
Therefore, to address \textbf{Req1}, INFv needs to be able to provide a mechanism to replace or extend application functionality with minimal impact and high coverage of devices.
In the literature such mechanisms have been provided by runtime patching techniques~\cite{mulliner_patchdroid:_2013} but targeted security patching in Android.

Inspired by the patching literature, in INFv we use binary patching techniques to provide functionality extension mechanisms similar to those of AOP.
More specifically, \emph{INFv applies a reversible patch to the OS (in this case Android) binaries in order to use a customized class loader and intercept method invocations}.
The binary patch is applied only once, when installing INFv.
In the case of Android, it targets the (\texttt{app\_process}), from which all launched app processes are forked (in a similar way to the Xposed framework~\cite{xposed}).
By redirecting invocations and using a custom class loader we are \emph{able to provide offloading capabilities in a transparent manner that does not require app developer intervention or repackaging the app}.
%Similar interception mechanisms have been ported to multiple versions of Android and are also available for other OSes (e.g., iOS~\cite{cydia}).
That said, as long as there are some common interfaces for defining hooks to intercept methods, our offloading solution should be agnostic of the OS in question or the app functionality extension mechanisms (e.g., Cydia for iOS~\cite{cydia}).
%Although on a higher level of abstraction this solution is still a common offloading architecture, designing such architecture from a patching perspective is technically challenging.

%In short, An object is a software bundle of related state and behavior. A class is a blueprint or prototype from which objects are created. An instance is a single and unique unit of a class.
%Example, we have a blueprint (class) represents student (object) with fields like name, age, course (class member). And we have 2 students here, Foo and Bob. So, Foo and Bob is 2 different instances of the class (Student class) that represent object (Student people).


\subsection{Functionality Offloading}

INFv receives the partition metadata (Sec. \ref{sec:partitions}) including a representation of the app and a description of the offloadable functionality.
For each partition's entry and exit points, INFv will allow the interception of its respective methods and offloading can occur depending on the current connectivity parameters (Sec. \ref{sec:decisions}).
%We will now focus on the offloading process, while in Section \ref{sec:decisions} we describe offloading decision model.

Once a target invocation is intercepted, our architecture is responsible of constructing and sending a message to the InfV network subsystem which executes it in the network in a transparent manner.
Offloading routing is done using the user, device, and app ids, along with the fully qualified method name and its arguments.
Additionally a version identifier is required to identify different versions of the same apps' functionality.
Likewise thread granularity approaches, our thread is suspended until it receives the method invocation result, although it can also resume if there is an incoming remote invocation that is supposed to execute on the same thread.

The InfV router subsystem will create and execute the class instance and respective methods in the network while also managing the instance state.
Even though most mobile applications are expected to be short-lived (often imposed by screen off events and CPU sleep mode), instance state maintenance is not trivial as state has to be kept while there are still references to the instance.
OO languages often provide mechanisms to deal/detect the garbage collection of objects~(e.g., Java's phantom/weak references and Objective C \texttt{dealloc} method), and so, network state can be invalidated upon such event.
In our solution, classes to be offloaded are replaced with lightweight mock objects \cite{objenesis}, which, on interception, work as proxy objects.
These objects are tracked using a custom weak identity hash map that allows the detection of de-referenced or garbage collected objects, which results in a state invalidation message being sent through the InfV network subsystem.
Additionally, application crashes or force quit also trigger state invalidation.
For simplicity, since the mobile devices can also go out of battery, state might be temporarily kept (e.g., saving VM state in non-volatile memory) in the network to provide better warranties for long lasting functionality.
More advanced mechanisms for distributed collection have been proposed in the past that target some of the aforementioned challenges \cite{abdullahi_garbage_1998}.  


\subsection{Runtime Decisions}
% \label{sec:decisions}

% \begin{figure}
%   \centering
%     \includegraphics[width=0.45\textwidth]{figures/architecture/metadata.pdf}
%     \caption{Design of INFv app analysis and partition functionality and metadata distribution.}
%     \label{fig:mobilearch}
% \end{figure}

When a mobile device with INFv installs an app, it retrieves from a repository the app partition's metadata (classes, execution and energy predictions) and app representation for each installed app.
The predicted metrics for the specific mobile device are then used as a function of the observed bandwidth, latency and device state (e.g., network type, screen state) for each remote execution call.
%While INFv collects some runtime metrics, such as the bandwidth (Mbps) -- $B$ -- and latency observed in each remote execution call, most of the networking monitoring and decisions occur within the network itself.
%Screen state and connection types are also used collected through Android event-driven events to get a better energy estimation.
%The decision to offload or not is performed on the mobile device.
A partition can be offloaded if the consumed energy and execution time are reduced when offloading.
When offloaded, energy consumption is composed mostly by the energy per transmitted bit for outgoing and ingoing state and most of the network monitoring and decisions occur within the network itself, which measures the latency in between nodes.
%Additionally, a threshold value (constant or from feedback loop) is used to account for variations between the estimated values and the observed ones (e.g., due to connectivity variations).

The Android platform already provides detailed diagnosis tools (i.e., android dumpsys) that provide many of the used metrics (e.g., CPU, screen state, foreground app, idle state, sensors, connectivity, battery state, etc) for each process.
Such reports can be collected daily and reported (when idle and on wifi) to our servers on two occasions, when the app is repeatadly performing worse than expected or randomly with a low probability of sending a daily report.
These metrics can be used to design a negative feedback loop and reduce the fluctuations between our estimations per device hardware and the observed values.

% \begin{align}\label{eq:decision}
% T_{res\_1}(\sum_{i=1}^{2}S_i/B + X_{off}) < X_{local},\\
% T_{res\_2}E_b\sum_{i=1}^{2}S_i < E_{local},\\
% X_{local} = K_1X_{off},\\
% E_{local} = K_2E_{est},\\
% \forall i \in [1,2], T_{res\_i} \geq 1,\\
% \forall i \in [1,2],K_i > 1,
% \end{align}


% %Other than just list of classes, partitions are shipped with the parameters for performing the decision to offload or not.
% Partition metadata parameters include server side estimations such as state -- $S_i$ -- execution time -- $X_{off}$ -- energy -- $E_{off}$ -- and ratios between mobile-network capabilities -- $K_1$,$K_2$.
% $S_i$ represents the size of the state, i.e., partition entry points method parameters -- $S_1$ --, the return -- $S_2$ -- and message headers to be sent in bits.
% The execution time ($X_{off}$),  and $S_i$ are estimated by instrumenting the apps in VMs in INFvs servers and repositories.
% We setup our VMs to simulate the lower bound resources available in a NFV network node \manote{what exactly are these?} to determine the functionality execution time ($X_{off}$), while energy consumption ($E_{est}$) is estimated per mobile device hardware.
% When not possible to estimate for a specific hardware (e.g., we lack energy measurements), we estimate $K_i$ ratios -- mobiles' energy ($K_2$) and execution time ($K_1$) -- based on their hardware specification (e.g., cpu cycles, radio, etc).
% Repository side $K_i$ estimated values are estimated once per mobile device hardware and kept in the INFv repository.
% %Another possible solution would consist of executing a benchmark algorithm on the mobile device to estimate these factors.






%\liang{any good solutions for this task? in the worst case, we still need to come up a hand waving solution :)}
%Consumption monitoring: the idea is monitoring the overall energy consumption by injecting a small function before a class is launched. The challenge is that the monitoring can be very expensive if we perform it at function level. Then you need to propose some heuristic to do the similar job in a cheap way. One idea is associating some weight with each node in the call graph and only keep those important (e.g., frequently called or most energy-consuming ones) in the limited cache. Evict them out if the cache is full, this can be justified by typical usage pattern since there is strong temporal and spatial locality in both user usage pattern and application call pattern (refer to the working set in OS cache). You can probably show the trade-off between the granularity and information loss. In general, I expect to see something that after reaching some points, increasing cache size only brings marginal improvement on precision.

%Enhanced model: mention that in the future, after a large deployment, we can resort to crowd-source model \cite{oliner_carat:_2013} to enhance the current solution. The crowd-source model can provide better precision with even cheaper monitoring cost.


\subsection{Network Execution}
In our current prototype the network INFv subsystem executes Java processes that use a custom class loader to load the apps' classes and reflection to invoke the requested methods.
Native execution is supported, provided that the class performing the Java Native Interfaces and the native binaries are offloaded as well (Sec. \ref{sec:limitations}).
Similarly to the app profiling, in our experimental setup, functionality was run within an Android x86 VM to provide better support for app functionality with dependencies on the Android framework.
Once launched the process remains mostly idle, listening for incoming requests from the mobile device and consuming few resources.
After executing the requests and if there are no remaining references to the offloaded instances and no interaction with the mobile device for a threshold period of time, the VM can be stopped. 
Although our solution has some dependencies on Android, as the offloading system is mostly Java it could be easily ported to run on a pure Java Virtual Machine (JVM).
%In Android, if this is run as an application, additional mechanisms are required to instrument the app lifecycle
In the future we would like to explore the possibility of creating a lighter Android Dalvik/ART VM capable of running over Linux containers/unikernels to reduce the resource footprint.

%============================================================
%============================================================
%============================================================




\section{Network Subsystem}
\label{sec:network}

\jbnote{Again, there is massive redundant text with this and the previous 2 sections now i think?}

We start this section with two fundamental control strategies, followed by a basic workload analysis on a service router, based on which we propose a proactive strategy to avoid computation congestion. Then we present the actual algorithm (C3PO) with implementation details.


\subsection{Two Basic Strategies}
\label{sec:strategy}

Service execution consumes both CPU and memory as well as other resources such as bandwidth. Herein we focus on the first two since they are usually the most dominant resources. The goal of load balancing is achieved by strategically drop or forward the computation task to some other nodes to avoid being overloaded. However, instead of distributing load uniformly over all available nodes, a server is preferred to be executed as close to a client as possible to minimize induced latency.

Centralized coordination is not ideal in a practical deployment (especially out of datacenters) due to the obvious reasons: 1) A central solver needs global knowledge of all the nodes in a network; 2) the optimal strategy needs to be calculated periodically given the dynamic nature of network and traffic; 3) there is a single point failure; 4) there might be only marginal improvement over a smartly designed heuristic. Therefore, we study two basic strategies in this paper.

\begin{itemize}

\item \textbf{Passive Control}: with this strategy, a node tries to execute as many services as possible before being overloaded. Whenever a service request arrives, it will be executed by default given enough resources. If the node is overloaded, the request will be passed to the next hop along the path to a server, or dropped if current node is already the last hop node in ISP networks.

\item \textbf{Proactive Control}: with this strategy, a node tries to execute services conservatively to avoid being overloaded. To do so, a node estimates request arrival rate with which it can further estimate the potential consumption. If the estimate shows that the node may be overloaded, it only executes some requests and forwards the rest to the next hop neighbor with the lightest load. This strategy requires exchanging state information within a node's one-hop neighborhood.

\end{itemize}

Because of its simple logic, passive strategy has a very straightforward implementation. Clients can benefit from minimized service latency given no nodes are overloaded, since a service gets executed immediately at an edge router. For proactive strategy, the implementation relies on how estimate is made which we will detail in the following. Despite of being conservative, we still aim to keep the latency and algorithmic complexity low.


\subsection{Workload Analysis}
\label{sec:workload}

A node $n$ receives service requests either from directly connected clients or neighbours. We assume that a node $n$ has CPU capacity $c'$ and memory capacity $m'$.
For a specific service $f_j$, we denote its average CPU and memory consumption as $c_j$ and $m_j$ respectively. In practice, both can be easily measured by tracking a service execution. We also assume the execution time of $f_j$ follows an exponential distribution with its mean value equal to $t_j$\jbnote{any cite that would justify this assumption? Would be nice if possible.}. The requests for service $f_j$ can be viewed as a Poisson processes with arrival rate $\lambda_j$. We can easily recognise that the process is a typical \textit{birth-death process}. Because the joint process of multiple Poisson processs is also Poisson, the aggregated requests of all services form another well-defined birth-death process with the birth rate as $\lambda = \sum_{\forall j} \lambda_j$ and death rate as $\mu = \sum_{\forall j} \frac{1}{t_j}$. We herein focus on this aggregate request stream.

To calculate average workload, for any given time, we need to estimate the average number of simultaneously running services on node $n$, denoted as $l$. This is equivalent to calculating the average queue length in a simple $M/M/1$ queueing system, where the clients in a queue represents the services running concurrently on a node by applying a multiprogramming model. Herein we consider a stable system where $\lambda < \mu$ to prevent a queue from growing infinitely long to overload a node. We will show later how a proactive strategy is able to keep the system stable.  We have assumed that one CPU is allocated for service execution hence we choose to use $M/M/1$ model in this paper to simplify the discussion. However the analysis can be easily extended to $M/M/C$ model to analyse a multi-core system.

Let $p_j$ denote the normalised popularity of $f_j$ derived from all the requests observed by $n$, then $p_j = \frac{\lambda_j}{\lambda}$ and note that $\sum_{\forall j} p_j = 1$ by definition. The average CPU consumption is $c'' = \sum_{\forall j} p_j \times c''_j$ and average memory consumption is  $m'' = \sum_{\forall j} p_j \times m''_j$. If we let $\rho = \frac{\lambda}{\mu}$ (i.e., utilisation rate), then we have $l = \frac{\rho}{1 - \rho}$ by applying a stationary analysis on $M/M/1$ model. Therefore we can calculate the overall workload induced by executing services in a straightforward way: namely $l \times c''$ for CPU load and $l \times m''$ for memory load. 


\subsection{Probabilistic Execution}
\label{sec:prob}

To avoid overloading a node, we need to make sure the workload is less than $n$'s actual capacity. As we have shown, workload is directly controlled by the queue length $l$, which can be further tuned by probabilistically selecting some requests in a stream to execute and forwarding the rest to the next hop. For each service request, if we let node $n$ execute a service with probability $q$, and $q \in [0,1]$ follows a uniform distribution. According to basic queueing theory, the resulting sub-process forms another well-defined birth-death process, with a new birth rate $q \times \lambda$ and the same death rate $\mu$. Therefore the new sub-process has a new utilisation rate equal to $q \times \rho$. To calculate $q$, we can simply perform the following derivations by letting the induced load (e.g., for CPU) $l \times c''$ less than the capacity $c'$.

\begin{align}
l \times c'' < c' & \Longrightarrow \frac{q \times \rho}{1 - q \times \rho} \times c'' < c' \\
& \Longrightarrow \rho \times q < \frac{c'}{c' + c''} \\
& \Longrightarrow  q < \frac{c'}{c' + c''} \times \frac{\mu}{\lambda}
\end{align}

The formula has a very intuitive explanation: if services can be executed faster on average (i.e., higher death rate $\mu$), node $n$ increases $q$ in order to serve more requests by maintaining a longer queue; otherwise $n$ decreases $q$ to reduce the queue length. If requests arrive faster (i.e., higher birth rate $\lambda$), the node also decreases $q$ to keep the number of simultaneously running services low. Similarly, we can perform the same calculations for memory constraint $m'$. Eventually, we set $q$ with the following formula.

\begin{align}
& q = \max\{ \min\{ \frac{c'}{c' + c''}, \frac{m'}{m' + m''} \} \times \frac{\mu}{\lambda}, 1\}
\label{eq:0}
\end{align}

The formula above essentially indicates that the final $q$ is decided by the first bottleneck in a system, either CPU or memory in our case. Also, $q$ is capped by $1$, indicating that an underutilised system will simply accept all the requests. 

%%%\liang{FIX: new thinking ... should $c'$ be updated to available resources every time I calculate $q$? In actual implementation, I maintain a queue of length of $x$, then my current hunch is that $x$ is parameter of sensitivity (or responsiveness) to flow dynamics (or changes in the request rates), namely the capability of smoothing jitters. Also, we use fix queue length instead of using fix window to prevent overflow when the rate is high, need to clarify.  Also, the problem of using fix time window is: setting window too large underestimate the jitter/changes, setting it too small overestimate the changes.}

%%%\liang{also need to mention, for passive, we keep forwarding to next-hop if every passing by router is busy, then drop at the last hop. We do so by presenting from forwarding too many times to increase latency and loops ... just need to clarify a bit.}

%%%\liang{In the algorithm design, need to use ARMA with exponential average to estimate CPU and Mem cost instead of maintaining the whole history.}




\subsection{Proactive Control - C3PO}
\label{sec:congestion}

We present an implementation of proactive control in Algorithm~\ref{algo:1}, namely \textit{C3PO} -- Computation Congestion Control (PrOactive). The algorithm consists of two major functions: \textbf{on\_arrival($\cdot$)} (line 1--10) is called whenever a service request arrives; and \textbf{on\_complete($\cdot$)} (line 12--21) is called whenever a service execution is completed. The notations used in the algorithm follow the same definition as those in the previous text. By keeping track of CPU usage $c''$, memory usage $m''$, execution rate $\mu$, and request arrival rate $\lambda$, the previous analysis shows how to control the workload by tuning execution probability $q$. However, maintaining a complete history of these statistics can be very expensive. In the actual implementation, we use four circular buffers of size $k$: 1) buf$_\lambda$ for the timestamps of the most recently arrived requests; 2) buf$_\mu$ for the execution time of the most recently finished services; 3) buf$_{c''}$ and 4) buf$_{m''}$ for CPU and memory usage of the most recently finished services.

\begin{algorithm}[!tb]
  \caption{C3PO - Proactive Computation Control}
  \label{algo:1}
  \begin{algorithmic}[1]
    \STATE{void \textbf{on\_arrival} (request $r$):}

    \STATE{\quad buf$_\lambda$[$i$] $\leftarrow$ timestamp ($r$)}

    \STATE{\quad $\lambda \leftarrow$ mean\_rate (buf$_\lambda$)}
    
    \STATE{\quad $\Delta \lambda \leftarrow$ max$(0, \lambda - \lambda')$}

    \STATE{\quad $\lambda \leftarrow \lambda + \Delta \lambda$}

    \STATE{\quad $q \leftarrow$ \textbf{eq.\ref{eq:0}} ($\lambda, \mu, c', c'', m', m''$)}
    
    \STATE{\quad \textbf{if} draw\_uniform ([0,1]) $ < q$ \textbf{then} execute ($r$)}
    
	\STATE{\quad \textbf{else} forward\_to\_lightest\_load\_node ($r$)}    
    
    \STATE{\quad $i \leftarrow (i+1)$ mod $k$}
    
    \STATE{\quad \textbf{if} $i == 0$ \textbf{then} $\lambda' \leftarrow 0.5 \times $($\lambda' + \lambda - \Delta \lambda$)}

	\STATE
	
	\STATE{void \textbf{on\_complete} (service $s$):}

	\STATE{\quad buf$_\mu$[$i$] $\leftarrow$ execution\_time ($s$)}
	\STATE{\quad buf$_{c''}$[$i$] $\leftarrow$ cpu\_consumption ($s$)}
	\STATE{\quad buf$_{m''}$[$i$] $\leftarrow$ memory\_consumption ($s$)}

	\STATE{\quad $i \leftarrow (i+1)$ mod $k$}
    
    \STATE{\quad \textbf{if} $i == 0$ \textbf{then}}
    \STATE{\quad \quad $\mu \leftarrow 0.5 \times $($\mu +$ mean(buf$_{\mu}$)$^{-1}$)}
    \STATE{\quad \quad $c'' \leftarrow 0.5 \times $($c'' +$ mean (buf$_{c''}$))}
    \STATE{\quad \quad $m'' \leftarrow 0.5 \times $($m'' +$ mean (buf$_{m''}$))}
    
    \STATE{\quad forward\_result (s)}
  \end{algorithmic}
  %%% \vskip -5mm
\end{algorithm}

With these four circular buffers, we can calculate the recent values of the parameters in eq.\ref{eq:0}. We decide to use fixed buffer instead of fixed time window to prevent the memory usage of Algorithm \ref{algo:1} from being subject to service arrival/completion rate. Parameter $k$ represents a trade-off between stability and responsiveness. Larger $k$ leads to more stable estimates whereas smaller $k$ indicates higher responsiveness of a strategy to the changes in two metrics (i.e., $\lambda$ and $\mu$). Line 2--6 calculate the execution probability $q$.
The algorithm also maintains a variable $\lambda'$ for the average arrival rate of previous $k$ requests, so that we can calculate the variation in $\lambda$ as $\Delta \lambda = \lambda - \lambda'$. It is definitely worth emphasising line 4 and 5: when $\Delta \lambda > 0$, it indicates an increase in request arrival rate, then C3PO will enter into conservative mode. In conservative mode, C3PO updates $q$ at line 6 by plugging $(\lambda + \Delta \lambda)$ as arrival rate in eq.\ref{eq:0} rather than plugging original $\lambda$. In such a way, C3PO "pessimistically" estimates the arrival rate will increase at the same rate $\Delta \lambda$ in a near future.
If $\Delta \lambda \leq 0$, C3PO operates in normal mode. In some sense, "being proactive" is achieved by "being conservative" when noticing a potential increase in resource consumption.

Although $\lambda$ needs to be calculated at every request arrival (line 3), we can optimise the performance by using another variable $x$ to keep track the sum of arrival intervals.
%%%namely $x \leftarrow \sum_{\forall j \neq i}($buf$_\lambda[(j-1)$ mod $k] -$ buf$_\lambda[j])$. Note head condition is handled by $j \neq i$. 
If we further let $y \leftarrow  \text{buf}_\lambda[(i+1) \text{ mod } k] - \text{buf}_\lambda[i]$ and $z \leftarrow \text{timestamp}(r) - \text{buf}_\lambda[(i-1) \text{ mod } k]$ before performing line 2, then mean rate can be calculated by $\lambda \leftarrow (x - y + z]) / (k - 1) $. Because all $x,y,z$ can be updated with $\mathcal{O}(1)$, this reduces the complexity of "mean\_rate" function from $\mathcal{O}(k)$ to $\mathcal{O}(1)$ by avoiding traversing through all the timestamps in buf$_\lambda$.
Other parameters except $\lambda$ are updated only periodically in both functions (line 10, 18-20). We apply an ARMA (AutoRegressive Moving Average) model with exponential mean when updating these parameters. Both history and recent measure are given the equal weight 0.5. 
To keep the code short and easy to understand, we did not perform further optimisations in Algorithm \ref{algo:1}.

==> sections/deprecated/old_design.tex <==
\section{Design Requirements and Challenges}
\label{sec:arch}

The overall INFv architecture is shown in Figure \ref{fig:architecture}.
The three different logical subsystems are separated by dotted lines.
First subsystem profiles apps to capture good offloading candidates based on their energy and computation characteristics then devises offloading strategies. 
The second subsystem runs both on top of a user device and its counterpart on a virtual machine on a generic machine in the network (NFV).
On user devices, it monitors devices properties (e.g., screen state, connectivity, latency, etc) and makes offloading decisions by using the strategy provided by the first subsystem. 
On network devices, it invokes the function calls and returns the results. 
Finally, the third subsystem runs on the network nodes and is responsible for caching functionality and balancing the computation load.

In the following sections we identify the design requirements and challenges. Then we present the overall system architecture to illustrate its basic functionality. 

\begin{figure}
  \centering
    \includegraphics[width=0.45\textwidth]{figures/architecture/overall.pdf}
    \caption{Design of INFv overall system.}
    \label{fig:architecture}
\end{figure}

%%% Some system requirements: non-intrusive, transparent to applications; compatible with current systems and networks; safe and efficient; robust regarding different failure modes; and etc.

%Mobile code offloading distribution design differs from that of a client/server paradigm since part of the client code is executed in the cloud.
%While mobile devices are mostly consumers of third-party data, offloading mobile functionality means that devices will act as both consumers of the functions output and producers of their respective inputs.
%These functions can make use of third-party services content as well.
%Our proposal regarding in-network functionality hosting can accommodate for both client and/or service functionality to be hosted on the network.
%It relies on three subsystems to handle functionality communication.

\subsection{Profiling Subsystem}
\label{sec:profiling}

In mobile code offloading, apps are typically partitioned into a set of functionality to execute locally and another to execute remotely.
Such system needs to detect good candidates to offload, e.g., based on energy consumption and execution time.
The selection is done via static and dynamic analysis on apps' behaviors (a.k.a., profiling apps).
%To assure that offloading an app does not consume more energy or takes longer than executing locally, apps need to be profiled.
Since profiling per se is energy consuming and can degrade devices' performance, we devise our first requirement:
\textbf{Req1)} \emph{App profiling should have minimal impact mobile device energy consumption and performance.}
In our design most of the profiled metrics and estimations are performed remotely (INFv servers) for a given mobile device.
%in INFvs' servers and the respective results are shipped to the devices in order to estimate the local parameters (i.e., execution time and energy consumption) required for offloading.

%Adittionally app analysis is also responsible for detecting functionality that should be executed locally and to approximate the existing estimations to the observed 

INFvs profiling subsystem consists of an app analysis cluster and repository containing these apps' partition functionality as well as their respective metadata.
This metadata includes the app representation (e.g., information regarding app structure and method invocations) and estimated resource usage (e.g., energy, execution time).
The app analysis cluster has a set of schedulers that launch VM instances to analyze apps then stores the respective results in the repository.
App analysis is done through static (i.e. parsing decompiled bytecode) and dynamic analysis of the apps.
% to retrieve functionality execution time, parameter state and energy consumption.
The first is used to retrieve the metadata app representation and do an initial prediction of possible partitions (e.g., pinning to execute locally functionality that uses devices hardware).
The second is used to benchmark app partitions and to retrieve functionality execution time, parameter state and energy consumption (i.e., partition's metadata), which is used for performing informed offloading decisions.

\subsection{Offloading Subsystem}

With the app behavior predictions and offloading strategy in place, an offloading subsystem is required for instrumenting and modifying app behavior to support offloading.
One of our design principles is to minimize the adoption barrier of the system, i.e., it should not impose any modifications on existing applications such as application repackaging, custom firmware flashing or custom app stores.
Therefore we devised our second requirement:
\textbf{Req2)} \emph{It must have minimal impact on the ecosystem.}
Mobile device users should be able to run unmodified apps downloaded from the official app stores.
Since we do not repackage existing apps to avoid introducing any difficulties in adopting our solution, remote resource execution should be done in an automated fashion and so we reach our third requirement.
\textbf{Req3)} \emph{It must enable apps to make use of remote resources in a transparent and efficient manner.}
With our design, the mobile device fetches the profiling information to perform offloading decisions without affecting user experience and performance.
%: \textbf{Req2)} \emph{Functionality should only be offloaded when its energy and execution time are reduced.}
As a result our design focuses on allowing the automation of the offloading process, without requiring programming frameworks or manual annotation of functionality.


%<<<<<<< HEAD
% \begin{figure}
%   \centering
%     \includegraphics[width=0.25\textwidth]{figures/architecture/mobile.pdf}
%     \caption{Design of INFv End Device system. The INFv monitor is a module that executes within apps and is responsible for monitoring app functionality. The INFv network is a separate process responsible for routing the monitor's offloading requests.}
%     \label{fig:mobilearch0}
% \end{figure}

%As shown in Figure \ref{fig:mobilearch0}, 
%The INFv mobile ecosystem consists of a stock mobile OS (discussion in Section \ref{sec:security}), an unmodified application to be offloaded and a per device INFv network stub. \liang{FIX: calling it network module is confusing ... would network stub make more sense?}\manote{i think stub makes sense here, good point.}
%The per device INFv network module is a standalone process responsible for the monitoring of installed apps and fecthing their potential partitions metadata.
%=======
\begin{figure}
  \centering
    \includegraphics[width=0.25\textwidth]{figures/architecture/mobile.pdf}
    \caption{Design of INFv End Device system. %The INFv monitor executes within apps and instruments app functionality. The INFv network is a separate process that routes offloading requests.
    }
    \label{fig:mobilearch0}
\end{figure}

As shown in Figure \ref{fig:mobilearch0}, the INFv mobile ecosystem consists of a stock mobile OS (discussion in Section \ref{sec:security}), an unmodified application to be offloaded and a per device INFv network stub. \liang{FIX: calling it network module is confusing ... would network stub make more sense?}\manote{i think stub makes sense here, good point.}
The per device INFv network module is a standalone process responsible for the monitoring of installed apps and fecthing their partitions metadata.
%>>>>>>> conext
It also handles the offloading requests originating and destined to the mobile device apps, abstracting the network interaction.
The INFv monitor is a binary patch applied to apps processes which provides the execution interception mechanisms.
%On installation, INFv modifies (one time patch) the process that is forked by all apps.
%This modification allows apps to load additional functionality on start.
%Other than execution interception mechanisms, INFv also loads information about possible app partitions (i.e., remote vs local functionality) and estimated energy and execution parameters.
Using the partitions metadata, i.e., resource usage estimations and functionality set to be offloaded, the INFv monitor can decide whether an app functionality should be offloaded or not reducing the overall energy consumption and execution time of the app.


\subsection{Network Subsystem}

Functionality execution consumes multiple resources on a network device, especially CPU cycles for computation intensive tasks. 
It introduces a new type of "congestion" in a network which we refer to as \textit{"computation congestion"}. 
Different from conventional traffic congestions which are avoided by the cooperation of both communication ends, in-network services do not necessarily impose a point-to-point paradigm.
Also different from the classic load balancing problem in the cloud, which often has a regular structure (i.e., regular network topology, central coordination, homogeneous configurations, uniform demands, and etc.), the situation in an ISP network is often more complicated.
So for the second subsystem we highlight the following design requirements:
\textbf{Req5)} \emph{It must support arbitrary network topologies and node heterogeneity.}
Not only can the ISPs topology be irregular when compared to the cloud, but it also has heterogeneous node configurations (including NFV nodes)\jbnote{citation?}.  
The functionality demand distribution can be highly skewed hence resources in a neighborhood needs to be well utilized, so we define our last requirement:
\textbf{Req6)} \emph{It must adapt to demand and balance load in the network.}
Additionally, as central coordination can incur extra costs (e.g., dedicated network services) and can reduce responsiveness of the nodes hosting these functionalities, our design will also be decentralized.
Next sections provides more details on each of INFv's subsystems.

The network subsystem is responsible for receiving clients' requests, performing workload balancing, and scheduling the execution of offloaded functionality.
This subsystem is fully decentralized and implements a ``computation congestion control'' algorithm that can pro-actively distribute functionality in a nodes' neighborhood.
The INFv mobile end system connects to the closest INFv-enabled network node by explicit registration. Service discovery can be done by using either a DNS-like service or ad-hoc discovery.
The connected node maintains a message queue system to deliver messages to and from the mobile device.
When a new offloading request arrives at the queue, based on the availability (cache) of the functionality and the current workload, the request may either be executed locally or offloaded to a neighbor. In both cases, a new VM should be spawned to execute the request.
This VM runs a lightweight process that loads the app functionality (e.g., classes, native binaries) and executes the request invocation call.


% \subsection{A Use Case of Face Detection App}
% \label{sec:usecase}

% An example of computation intensive applications are those that process images and video, one such case is the detection of human faces.
% Detecting faces in images is useful for cropping and adjusting images (e.g., red-eye correction and tone balance) and most mobile OSes already provide face detection apis (e.g., Android\cite{fddroid} and iOS\cite{fdios}). 
% %A face detection application that uses this apis generally retrieves images (or videos) from the camera or a local photo library and makes use of the OS apis to detect the faces.
% %These apis return the coordinates and orientation of faces (and other features such as mouth and eyes) in a supplied image.
% %Since image processing libraries are computationally intensive, executing them over a more powerful machine can provide energy and performance benefits.
% In a device with INFv, when such app is installed the device also downloads some metadata describing its estimated resource usage and a strategy to optimize it (partition metadata).
% When the face detection app executes, its behavior is transparently modified so that, for example, when a user uses its camera to take a picture, INFv estimates the energy savings and finds a proximate low-latency network node with the required functionality (partition functionality) to execute the time and energy consuming computations.
% This network node then returns the coordinates and orientation of faces (and other features such as mouth and eyes) in the supplied image to the mobile device.
% As an end result, not only the app provides the same functionality faster due to the disparity between the mobile device hardware and that of the network node, but also consuming less energy as the mobile device app is mostly idle during offloading.
% These apis represent a very interesting case because they also require the transmission of images, which tend to be on a order of MBs.
% Therefore they demonstrate the offloading trade off between the communication time and computational speed up and have thus become a common target of mobile code offloading research (e.g., \cite{Shi:2014:CCO:2632951.2632958}).
% %%% In section \ref{sec:evaluation:offloading} we depict these trade-offs for two apps (including face detection) using our INFv architecture and further demonstrate the impact of the app partition decisions over different types of connectivity (i.e., wifi and 3G).

%============================================================
%============================================================
%============================================================


